Satisfying Rationality Postulates of Structured Argumentation Through Deductive Support -- Technical Report

ASPIC-style structured argumentation frameworks provide a formal basis for reasoning in artificial intelligence by combining internal argument structure with abstract argumentation semantics. A key challenge in these frameworks is ensuring compliance with five critical rationality postulates: closure, direct consistency, indirect consistency, non-interference, and crash-resistance. Recent approaches, including ASPIC$^{\ominus}$ and Deductive ASPIC$-$, have made significant progress but fall short of meeting all postulates simultaneously under a credulous semantics (e.g. preferred) in the presence of undercuts. This paper introduces Deductive ASPIC$^{\ominus}$, a novel framework that integrates gen-rebuttals from ASPIC$^{\ominus}$ with the Joint Support Bipolar Argumentation Frameworks (JSBAFs) of Deductive ASPIC$-$, incorporating preferences. We show that Deductive ASPIC$^{\ominus}$ satisfies all five rationality postulates under a version of preferred semantics. This work opens new avenues for further research on robust and logically sound structured argumentation systems.

==> jsbaf_tr.tex <==
%
To prove Theorem~\ref{Theo:PreferredExistence}, we need to show that admissible labelings always exist and that it is possible to choose a maximal adbmissible labeling even in the case of a JSBAF with an infinite number of arguments.\footnote{
%
Since we want to base the strict rules of our version of ASPIC on some underlying logic, we will usually end up with infinitely many arguments in our JSBAFs.
}
%
For the first part, we can define a family of labelings which labels precisely the strict arguments of a JSBAF as \In, labels all arguments \Out that are legally \Out as a result from accepting the strict arguments and labels all the remaining arguments \Undec.
%
We can then show that in every JSBAF, the labeling resulting from this approach is an admissible labeling, meaning $adm(\mathcal{J})\neq\emptyset$.
%
For the second part, we can use Zorn's Lemma\footnote{
%
Zorn's Lemma states that if $X$ is a partially ordered set \suchthat every chain in $X$ has an upper bound, then $X$ contains a maximal element. It follows from the Axiom of Choice.
}
%
 to show that $adm(\mathcal{J})$ contains a maximal element.
%

\textbf{Marcos: Der Rest von diesem Abschnitt braucht meines Erachtens nicht im Paper zu sein, sondern nur im Technical Report.}

%
We begin with the definition of a \emph{strict including minimal labeling} (SIM) of a JSBAF:
%
\begin{definition}
For any JSBAF \JSBAF, $SIM_{\mathcal{J}}$ is defined as:
\begin{enumerate}
\item {$in(SIM_{\mathcal{J}})=STR_{\mathcal{J}}$}
\item {
\(\begin{aligned}[t]
O_0
&=\big{\{ }a\in \mathcal{A}\mid(b,a)\in {\rightarrow},b\in STR_{\mathcal{J}}\big{\} }\\
O_{n+1}
&= O_n \cup \big{\{ }A\in \mathcal{A}\mid (S,b)\in {\Rightarrow}, a\in S, b\in O_n,\\
&\hspace{2.8cm}S\backslash\{a\}\subseteq STR_{\mathcal{J}}\big{\} }\end{aligned}
\\
out(SIM_{\mathcal{J}})=\bigcup\limits_{i\geq 0} O_i
$}
\item {$undec(SIM_{\mathcal{J}})=Args\:\backslash\:\big(in(SIM_{\mathcal{J}})\cup out(SIM_{\mathcal{J}})\big)$}
\end{enumerate}
\end{definition}



==> preliminaries.tex <==
We fix a set $\mathcal{F}$ of well-founded formulas closed under negation $\lnot$ and conjunction $\wedge$ and with $\bot,\top\in\mathcal{F}$ being the only formulas denoting truth values false and true.\footnote{
Throughout this paper, one may think of Propositional Logic or First Order Logic to get an idea of the logical languages we want to cover with our definitions.}
%
We write $\phi,\psi$ for single formulas and $\Gamma,\Delta$ for sets of formulas.
%
We define $Atoms:\mathcal{F}\mapsto 2^{\mathcal{F}}\backslash\{\bot,\top\}$ to be a function mapping formulas to atomic formulas and write $\phi||\psi$ to say that $Atoms(\phi)\cap Atoms(\psi)=\emptyset$, as well as $\Gamma||\Delta$ to say that $Atoms(\phi)\cap Atoms(\psi)=\emptyset$ for all $\phi\in\Gamma$ and $\psi\in\Delta$.
%
Let $\Gamma=\{\phi_0,...,\phi_n\}$ be a set of formulas \st $\phi_i\leq_l\phi_{i+1}$ according to some total ordering $\leq_l$.
%
As a shorthand notation, we define $\bigwedge\Gamma$ recursively as $\bigwedge\Gamma=\phi_0$ if $n=0$ and $\bigwedge\Gamma=\phi_0\wedge\bigwedge\{\phi_1,...,\phi_n\}$ otherwise.
%
Furthermore, we write $\phi=-\psi$ to indicate that either $\phi=\lnot\psi$ or $\lnot\phi=\psi$ and $\Delta=-\Gamma$ to indicate that either $\bigwedge\Gamma=\lnot\bigwedge\Delta$ or $\lnot\bigwedge\Gamma=\bigwedge\Delta$.
%
Let $\mathcal{I}$ be a class of objects called interpretations, which we denote as $I$ and let $\isModelOf\subseteq\mathcal{F}\times\mathcal{I}$.
%
We call $I$ a model of $\phi$ if $I\isModelOf\phi$ and a model of $\Gamma$ if $I\isModelOf\phi$ for all $\phi\in\Gamma$.
%
We say that $\Gamma$ is satisfiable if there exists $I\in\mathcal{I}$ \st $I\isModelOf\Gamma$, otherwise we call $\Gamma$ unsatisfiable.
%
We call $\Gamma$ (or $\phi$) tautological if $I\isModelOf\Gamma$ ($I\isModelOf\phi$) for all $I$.
%
For any $\phi,\psi$ and any $I$ we define $I\isModelOf\phi$ iff not $I\isModelOf\lnot\phi$.
%
Furthermore, we define $I\isModelOf\phi\wedge\phi$ iff $I\isModelOf\phi$ and $I\isModelOf\psi$.
%
For any $I_1,I_2$, if $I_1\isModelOf\phi$, $I_2\isModelOf\psi$ and $\phi||\psi$, we assume that there exists $I$ \st $I\isModelOf\phi$ and $I\isModelOf\psi$.
%
We define the consequence relation $\entails\subseteq 2^{\mathcal{F}}\times\mathcal{F}$ as $\Gamma\entails\phi$ iff for all $I$, if $I\isModelOf\Gamma$, then $I\isModelOf\phi$.
%
Note that by this definition, $\Gamma\entails\phi$ implies $\Gamma\cup\{\psi\}\entails\phi$.
%
The basis of our version of ASPIC will be a \emph{classical logic}, $\mathcal{CL}$, which we define as the tuple \ClassLog.

Given some $\mathcal{CL}$, we define a defeasible theory as the tuple \DefTheo where $AX\subseteq\mathcal{F}$ is a satisfiable set which we call axioms, $R_d$ is a set of defeasible inference rules of the form $\phi_0,...,\phi_m\Rightarrow\phi$, $n:R_d\mapsto \mathcal{F}$ is a (partial) naming function and $\leq_r\subseteq R_d\times R_d$ is a partial preorder called preferences order.
%
The argumentation system (AS for short) corresponding to $DT$ is the tuple \AS where $R_s=R_s^{AX}\cup R_s^{\vDash}$ is a set of strict inference rules with $R_s^{AX}=\{\rightarrow\phi\mid\phi\in AX\}$ and $R_s^{\vDash}=\{\phi_0,...,\phi_m\rightarrow\phi\mid\{\phi_0,...,\phi_m\}\vDash_C\phi\}$.
%
When the distinction between strict and defeasible rules is not relevant, we use $\rightsquigarrow$ and mean by that either $\rightarrow$ or $\Rightarrow$.
%
Arguments based on $AS$ are defined recursively and denoted with lower case letters $a,b,c$, while sets of arguments are denoted with capital letters $A,B,C$.
%
$a$ is an argument iff it is of the form $a=a_0,...,a_m\rightsquigarrow\phi$, where $a_0,...,a_m$ are arguments based on $AS$, $\phi$ is the conclusion of $a$, denoted $a^C$, and there exists a strict or defeasible rule of the form $a_0^C,...,a_m^C\rightsquigarrow\phi$.
%
For any set of arguments $A$, we define its conclusions as $A^C=\{a^C\mid a\in A\}$.
%
We say $a_0^C,...,a_m^C\rightarrow\phi$ is the top-rule of $a$, denoted $TR(a)$.
%
The defeasible rules of $a$ are defined recursively as $DR(a)=DR(a_0)\cup ...\cup DR(a_m)\cup \{TR(a)\}$ if $TR(a)\in R_d$ and $DR(a)=DR(a_0)\cup ...\cup DR(a_m)$ otherwise.
%
The sub-arguments of $a$ are $Sub(a)=Sub(a_0)\cup...\cup Sub(a_m)\cup\{a\}$.
If $a$ is of the form $a=a_0,...,a_m\rightsquigarrow\phi$ we call $\{a_0,...,a_m\}$ the direct sub-arguments of $a$.
%
We denote the arguments that can be constructed based on some $AS$ by $Args(AS)$.
%
We call $a$ defeasible if $DR(a)\neq\emptyset$ and strict otherwise.
%
We say $a$ is inconsistent if there is $\Gamma\subseteq Sub(a)^C$ \st $\Gamma$ is inconsistent, otherwise $a$ is consistent.
%
We call $AS$ inconsistent if there are strict arguments $a,b$ \st $a^C=-b^C$ and consistent otherwise.
%
Throughout this paper we only deal with consistent $AS$.
%
We say that $a$ undercuts $b$ iff there is $b'\in Sub(b)$ with $TR(b')=r\in R_d$ and $a^c=-n(r)$.
%
We use the notion of \emph{gen-rebuts} taken from Heyninck~and~Straßer~\cite{Heyninck2017:RevisitingUnrestrictedRebutPreferences} and say that $a$ gen-rebuts $b$ iff $b$ is defeasible and there is $\Gamma\subseteq Sub(b)^C$ \st $a^C=-\bigwedge\Gamma$.
%
We consider the elitist weakest link principle to lift preferences between defeasible rules to preferences over arguments, denoted by the relation $\preceq\subseteq Args(AS)\times Args(AS)$.\footnote{
We write $a\prec b$ to abbreviate $a\preceq b$ and $b\not\preceq a$.}
%
Let $a,b$ be arguments.
%
If $a$ is strict, then we define $a\not\preceq b$, if $b$ is strict and $a$ is not strict, we define $a\preceq b$ and if neither $a$ nor $b$ are strict, we define $a\preceq b$ iff $\exists r_a\in DR(a)$ \st $\forall r_b\in DR(B)$, $r_a\leq_d r_b$.
%
We say that $a$ \emph{defeats} $b$ if $a$ undercuts $b$ or if $a$ gen-rebuts $b$ and $a\not\prec b$.

Let \ASOne,\ASTwo be two AS.
%
We define the union of $AS_1,AS_2$ as $AS_+=(R_s^{AX_1}\cup R_s^{AX_2}\cup R_s^{\vDash},R_{d_1}\cup R_{d_2},n_1\cup n_2,\leq_1\cup \leq_2)$.
%
